Computational Aspects of Dependence Logic

In this thesis (modal) dependence logic is investigated. It was introduced in 2007 by Jouko V\"a\"aan\"anen as an extension of first-order (resp. modal) logic by the dependence operator =(). For first-order (resp. propositional) variables x_1,...,x_n, =(x_1,...,x_n) intuitively states that the value of x_n is determined by those of x_1,...,x_n-1. We consider fragments of modal dependence logic obtained by restricting the set of allowed modal and propositional connectives. We classify these fragments with respect to the complexity of their satisfiability and model-checking problems. For satisfiability we obtain complexity degrees from P over NP, Sigma_P^2 and PSPACE up to NEXP, while for model-checking we only classify the fragments with respect to their tractability, i.e. we either show NP-completeness or containment in P. We then study the extension of modal dependence logic by intuitionistic implication. For this extension we again classify the complexity of the model-checking problem for its fragments. Here we obtain complexity degrees from P over NP and coNP up to PSPACE. Finally, we analyze first-order dependence logic, independence-friendly logic and their two-variable fragments. We prove that satisfiability for two-variable dependence logic is NEXP-complete, whereas for two-variable independence-friendly logic it is undecidable; and use this to prove that the latter is also more expressive than the former.

==> chapters/bd.tex <==
% % % \begin{definition}[Syntax of \bd, \bbd, \rbd, \abd]\label{def logics}
% % % The logic \bd is defined by the following grammar:
% % % \[\begin{array}{lcl}
% % % \phi &\ddfn& x_1=x_2 \mid \neg\, x_1=x_2\mid R(x_1,\dots,x_n)\mid \neg R(x_1,\dots,x_n) \mid \\
% % % && \alpha \mid \neg\alpha \mid \dep[x_1,\dots,x_n, \alpha] \mid\\
% % % &&\phi \vee \phi \mid \phi \wedge \phi \mid \forall x \phi \mid \exists x \phi \mid \exists \alpha \phi
% % % \end{array}\]
% % % where $x, x_1,\dots, x_n$ denote first-order variables and $\alpha$ denotes a Boolean variable.
% % % 
% % % \bbd is the restriction of \bd to formulas
% % % \begin{itemize}
% % %  \item in which for every subformula of the form
% % % \[\forall x\big(\dots\exists y\big(\dots \dep[x_1,\dots,x_n,\alpha]\dots\big)\dots\big)\]
% % % it holds that $x\in\{x_1,\dots,x_n\}$, i.e.~whenever a dependence atom occurs inside the scope of an existential first-order quantifier it has to have every variable, which is universally quantified before the existential quantifier, in its precondition; or in other words, if a dependence atom $\dep[x_1,\dots,x_n,\alpha]$ occurs inside an existential first-order quantifier $\exists y$ then $\alpha$ must be allowed to depend on everything that $y$ depends on, and
% % %  \item without \emph{requantification} of variables that are required to occur in dependence atoms by the first rule, i.e.~there is no subformula of the form
% % % \[\forall x\big(\dots\exists y\big(\dots \forall x\big(\dots \dep[x_1,\dots,x_n,\alpha]\dots\big)\dots\big)\dots\big).\]
% % % \end{itemize}
% % % % \bbd is defined as \bd but $\phi ::= \forall x \phi$ is replaced by $\phi ::= \forall x \phi'$, where $\phi'$ is generated from $\phi$ by replacing each dependence atom $d:=\dep[x_{j_1},\dots,x_{j_n},\alpha]$ with
% % % % \[\left\{
% % % % \begin{array}{ll}
% % % % \dep[x,x_{j_1},\dots,x_{j_n},\alpha]&\text{if there is $\exists y \psi\in\sub{\phi}$ s.t.~$d$ occurs inside $\psi$}\\
% % % % d&\text{else}
% % % % \end{array}
% % % % \right.\]
% % % 
% % % \rbd is the restriction of \bd to formulas where no dependence atom occurs inside the scope of an existential first-order quantifier.
% % % % \rbd is the restriction of \bd where the rule $\phi::= \exists x \phi$ may only be applied if $\phi$ does not contain a dependence atom.
% % % 
% % % \abd is the restriction of \bd to formulas without existential quantification of first-order variables.
% % % \end{definition}
% % % 
% % % \begin{note}\label{bd subsets}
% % % $\abd\subsetneqq \rbd\subsetneqq \bbd\subsetneqq \bd$.
% % % \end{note}
% % 
% % 
% % % In order to define the semantics of $\bd$ and $\fopocp$ later, we first need to
% % % define the concept of a \emph{team}. Let $\mA$ be a model with the domain $A$.
% % % {\em Assignments} over $\mA$
% % % are finite functions that map first-order variables to elements of $A$ and Boolean variables to elements of $\{\bot,\top\}$. 
% % % We use $\alpha,\beta,\dots$ to denote Boolean variables and $x,y,\dots$ to denote first-order variables. Notice that Boolean variables are never assigned a value from the domain and first-order variables are never assigned a value $\bot$ or $\top$. 
% % % The value of a term $t$
% % % in an assignment $s$ is denoted by $t^{\mA}\langle s\rangle$.
% % % If $s$ is an assignment, $\chi$ a Boolean or first-order variable,  and $a\in A\cup\{\bot,\top\}$, then $s(a/\chi)$ denotes the 
% % % assignment (with the domain $\dom s\cup \{\chi\}$)  which agrees with $s$
% % % everywhere except that it maps $\chi$ to $a$.
% % 
% % % Let $A$ be a set and $\{x_1,\ldots,x_n,\alpha_1,\dots,\alpha_m\}$ a finite (possibly empty) set  of
% % % variables. 
% % %  A {\em team} $X$ of $A$ with the domain
% % % $\dom X=\{x_1,\ldots,x_n,\alpha_1,\dots,\alpha_m\}$ is any set of allowed assignments from the variables
% % % $\{x_1,\ldots,x_k,\alpha_1,\dots,\alpha_m\}$ into the set $A\cup\{\bot,\top\}$.
% % %We denote by $\rel(X)$ the
% % %$k$-ary relation of $A$ corresponding to $X$ 
% % %\[\rel(X)=\{(s(x_1),\ldots,s(x_k)) \mid s\in X \}.  \]
% % 
% % % If $X$ is a team of $A$,
% % % $F\colon X\rightarrow A$, $G\colon X\rightarrow \{\bot,\top\}$, we use $X(F/x)$ to denote the team
% % % \[\{s(F(s)/x) \mid s\in X \},\]
% % % $X(G/\alpha)$ to denote the team
% % % \[\{s(G(s)/\alpha) \mid s\in X \},\]
% % % $X(A/x)$ for the team
% % % \[\{s (a/x)\mid s\in X\ \textrm{and}\ a\in A \}\]
% % % and $X(A/\alpha)$ for the team
% % % \[\{s (a/\alpha) \mid s\in X\ \textrm{and}\ a\in \{\bot,\top\} \}.\]
% % 
% % % For a set $W\subseteq \dom X$ we call $F$ \emph{$W$-independent} (resp.~\emph{$W$-determined}) if for all $s,s' \in X$, with $s(\chi)=s'(\chi)$ for all $\chi\in \dom X \setminus W$ (resp.~for all $\chi\in W$), we have that $F(s)=F(s')$.
% % 
% % % \begin{definition}[Semantics of \bd]\label{semantics of bd}
% % % Let $\mA$ be a model and $X$ a team. The satisfaction relation $\mA\models_X\phi$ is defined as follows.
% % % \begin{align*}
% % % \mA\models_X l &\quad\Leftrightarrow\quad \forall s\in X: \mA,s\models_\fo l \text{ where $l$ is a first-order literal}\\
% % % \mA\models_X \alpha &\quad\Leftrightarrow\quad \forall s\in X: s(\alpha)=\top\\
% % % \mA\models_X \neg\alpha &\quad\Leftrightarrow\quad \forall s\in X: s(\alpha)=\bot\\
% % % \mA\models_X \phi\wedge\psi &\quad\Leftrightarrow\quad \mA\models_X \phi \text{ and } \mA\models_X \psi\\
% % % \mA\models_X \phi\vee\psi &\quad\Leftrightarrow\quad \mA\models_Y \phi \text{ and } \mA\models_Z \psi \text{ for some }Y\cup Z=X\\
% % % \mA\models_X \dep[\vec{x},\alpha]&\quad\Leftrightarrow\quad \forall s,s'\in X: s(\vec{x})=s'(\vec{x}) \text{ implies } s(\alpha)=s'(\alpha)\\
% % % \mA \models_X \exists x \psi &\quad\Leftrightarrow\quad \mA \models _{X(F/x)} \psi \text{ for some } F\colon X\to A\\
% % % \mA \models_X \forall x\psi&\quad\Leftrightarrow\quad \mA \models _{X(A/x)} \psi\\
% % % \mA \models_X \exists \alpha \psi &\quad\Leftrightarrow\quad \mA \models _{X(F/\alpha)} \psi \text{ for some } F\colon X\to \{\top,\bot\}\\
% % % % \mA \models_X \forall \alpha \psi &\quad\Leftrightarrow\quad \mA \models _{X(A/\alpha)} \psi
% % % \end{align*}
% % % \end{definition}


% % % \begin{definition}\label{logics-equivalence}
% % % Let $\LL$ and $\LL'$ be logics. Then we say that $\LL'$ is \emph{at least as expressive} as $\LL$ ($\LL\leqq \LL'$) iff for all sentences $\phi \in \LL$ there is a $\phi'\in \LL'$ such that for all structures $\mA$ it holds that $\mA\models \phi$ iff $\mA\models \phi'$.
% % % We say $\LL$ and $\LL'$ are \emph{equivalent} ($\LL \equiv \LL'$) iff $\LL\leqq \LL'$ and $\LL'\leqq\LL$.
% % % \end{definition}



% % % In \cite[p.~]{va07} V\"a\"an\"anen defines \emph{Dependence-friendly logic ($\df\ff$)} which is equivalent to Dependence logic but closer to Independence-friendly-logic in notation. In the same way it is possible to introduce a \emph{Boolean Dependence-friendly logic ($\bd\ff$)}.
% % % \begin{definition}[Syntax of \bd\ff, \bbd\ff, \rbd\ff, \abd\ff]\label{def bdf logics}
% % % The logic \bd\ff is defined by the following grammar:
% % % \[\begin{array}{lcl}
% % % \phi &\ddfn& x_1=x_2 \mid \neg\, x_1=x_2\mid R(x_1,\dots,x_n)\mid \neg R(x_1,\dots,x_n) \mid \\
% % % && \alpha \mid \neg\alpha \mid \exists\alpha\dof{x_1,\dots,x_n}\phi\\
% % % &&\phi \vee \phi \mid \phi \wedge \phi \mid \forall x \phi \mid \exists x \phi
% % % \end{array}\]
% % % where $x, x_1,\dots, x_n$ denote first-order variables and $\alpha$ denotes a Boolean variable.
% % % Note that we do not allow the plain existential Boolean quantifier $\exists \alpha$ here. This is, however, not a loss of generality since $\exists\alpha \,\phi(\alpha) \ \equiv\ \exists\alpha\dof{\fr{\phi}} \,\phi(\alpha)$ for all formulas $\phi$.
% % % 
% % % \bbd\ff is the restriction of \bd\ff to formulas
% % % \begin{itemize}
% % %  \item in which for every subformula of the form
% % % \[\forall x\big(\dots\exists y\big(\dots \exists\alpha\dof{x_1,\dots,x_n}\dots\big)\dots\big)\]
% % % it holds that $x\in\{x_1,\dots,x_n\}$, i.e.~%
% % % % whenever a Boolean quantifier occurs inside the scope of an existential first-order quantifier it must be allowed to depend on every variable, which is universally quantified before the existential first-order quantifier; or in other words,
% % % if a Boolean quantifier $\exists \alpha\dof{x_1,\dots,x_n}$ occurs inside an existential first-order quantifier $\exists y$ then $\alpha$ must be allowed to depend on everything that $y$ depends on, and
% % %  \item without \emph{requantification} of variables that are required to occur in Boolean quantifiers by the first rule, i.e.~there is no subformula of the form
% % % \[\forall x\big(\dots\exists y\big(\dots \forall x\big(\dots \exists\alpha\dof{x_1,\dots,x_n}\dots\big)\dots\big)\dots\big).\]
% % % \end{itemize}
% % % % \bbd is defined as \bd but $\phi ::= \forall x \phi$ is replaced by $\phi ::= \forall x \phi'$, where $\phi'$ is generated from $\phi$ by replacing each dependence atom $d:=\dep[x_{j_1},\dots,x_{j_n},\alpha]$ with
% % % % \[\left\{
% % % % \begin{array}{ll}
% % % % \dep[x,x_{j_1},\dots,x_{j_n},\alpha]&\text{if there is $\exists y \psi\in\sub{\phi}$ s.t.~$d$ occurs inside $\psi$}\\
% % % % d&\text{else}
% % % % \end{array}
% % % % \right.\]
% % % 
% % % \rbd\ff is the restriction of \bd\ff to formulas where no Boolean quantifier occurs inside the scope of an existential first-order quantifier.
% % % % \rbd is the restriction of \bd where the rule $\phi::= \exists x \phi$ may only be applied if $\phi$ does not contain a dependence atom.
% % % 
% % % \abd\ff is the restriction of \bd\ff to formulas without existential quantification of first-order variables.
% % % \end{definition}
% % % 
% % % Note that for $\rbd\ff$ we have forbidden \emph{even unrestricted} Boolean quantifiers to occur inside existential first-order quantifiers. They can, however, be simulated because
% % % \[\exists\alpha\,\phi(\alpha)\ \equiv\ \phi(\true)\vee\phi(\false)\]
% % % for all $\phi\in\bd$ such that $\phi$ does not contain dependence atoms.
% % % 
% % % 
% % % \begin{definition}[Semantics of \bd\ff]\label{semantics of bdf}
% % % The satisfaction relation $\mA\models_X\phi$ is defined as for $\bd$, with the following addition:
% % % \[\mA \models_X \exists \alpha \dof{x_1,\dots,x_n} \psi \quad\Leftrightarrow\quad \parbox[t]{7cm}{$\mA \models _{X(F/\alpha)} \psi$ for some $F\colon X\to \{\top,\bot\}$ such that $F$ is $\{x_1,\dots,x_n\}$-determined.}\]
% % % \end{definition}
% % % 
% % % 
% % % The following \lcnamecref{d-df} is the \bd analog of \cite[Proposition~3.44]{va07}.
% % % \begin{proposition}\label{d-df}
% % % \begin{enumerate}
% % %  \item Let $\phi\in\bd$ (resp.~$\bbd$, $\rbd$, $\abd$). Then there is a formula $\phi^*\in\bd\ff$ (resp.~$\bbd\ff$, $\rbd\ff$, $\abd\ff$) such that for all structures $\mA$ and teams $X$ it holds that
% % % \[\mA\models_X \phi \quad\text{iff}\quad \mA\models_X\phi^*.\]
% % %  \item Let $\phi\in\bd\ff$ (resp.~$\bbd\ff$, $\rbd\ff$, $\abd\ff$). Then there is a formula $\phi^{**}\in\bd$ (resp.~$\bbd$, $\rbd$, $\abd$) such that for all structures $\mA$ and teams $X$ it holds that
% % % \[\mA\models_X \phi \quad\text{iff}\quad \mA\models_X\phi^{**}.\]
% % % \end{enumerate}
% % % 
% % % As a special case, the above implies $\bd\equiv \bd\ff$ (resp.~$\bbd\equiv\bbd\ff$, $\rbd\equiv\rbd\ff$, $\abd\equiv\abd\ff$).
% % % \end{proposition}
% % % \begin{proof}
% % % \begin{enumerate}
% % %  \item $\phi^{*}$ is generated from $\phi$ by replacing each dependence atom $\dep[x_1,\dots,x_n,\alpha]$ in $\phi$ with
% % % \[\exists\alpha'\dof{x_1,\dots,x_n}\,(\alpha'=\alpha).\]
% % %  \item $\phi^{**}$ is generated from $\phi$ by replacing each subformula $\exists \alpha\dof{x_1,\dots,x_n} \psi$ in $\phi$ with
% % % \[\exists\alpha\,\big(\dep[x_1,\dots,x_n,\alpha]\wedge \psi\big).\]
% % % \end{enumerate}
% % % \end{proof}
% % % 
% % % 
% % % 
% % % \begin{definition}[Syntax of \pocfo, \fopoc, \fopocp]
% % % The logic \pocfo is the set of all formulas
% % % \[\underbrace{
% % % \poc[cccc]{
% % % \forall x_{11}&\dots&\forall x_{1n}&\exists \alpha_1\\
% % % \vdots&&\vdots&\vdots\\
% % % \forall x_{m1}&\dots&\forall x_{mn}&\exists \alpha_m}
% % % }_{=: N^m_n \vec x_1\dots \vec x_m \alpha_1\dots \alpha_m} \phi\]
% % % with $\phi \in \fo$.
% % % 
% % % The logic \fopocp is defined by the following grammar:
% % % \[\begin{array}{lcl}
% % % \phi &::=& \alpha \mid \neg\alpha \mid x_1=x_2 \mid \neg x_1=x_2\mid R\vec x\mid \neg R\vec x \mid\\
% % % &&\phi \vee \phi \mid \phi \wedge \phi \mid \forall x \phi \mid \exists x \phi\\
% % % && N^m_n \vec x_1\dots \vec x_m \alpha_1\dots \alpha_m \phi
% % % \end{array}\]
% % % where $x, x_1,\dots, x_n$ denote first-order variables, $N^m_n \vec x_1\dots \vec x_m \alpha_1\dots \alpha_m$ is a partially ordered connective as defined above.
% % % %and $\breve{N}^m_n \vec x_1\dots \vec x_m \alpha_1\dots \alpha_m := \neg N^m_n \vec x_1\dots \vec x_m \alpha_1\dots \alpha_m$.
% % % 
% % % \fopoc is defined as the negation closure of \fopocp.
% % % \end{definition}
% % % 
% % % \begin{definition}[Semantics of \fopocp]\label{semantics fopocp}
% % % Let $\mA$ be a model (over the universe $A$) and $X$ a team. The satisfaction relation $\mA\models_X\phi$ is defined as follows. Here, we assume w.l.o.g.~that no variable is \emph{requantified} in $\phi$, i.e.~there is no subformula of the form $\exists x \psi$ (or $\forall x\psi$) with a subformula of the form $\exists x \theta$ in it.
% % % \[\begin{array}{lcl}
% % % \mA\models_X l &\Leftrightarrow &\forall s\in X: \mA,s\models_\fo l \text{ where $l$ is a first-order literal}\\
% % % \mA\models_X \alpha &\Leftrightarrow& \forall s\in X: s(\alpha)=\top \text{ where $\alpha$ is a Boolean variable}\\
% % % \mA\models_X \neg\alpha &\Leftrightarrow& \forall s\in X: s(\alpha)=\bot  \text{ where $\alpha$ is a Boolean variable}\\
% % % \mA\models_X \phi\wedge\psi &\Leftrightarrow& \mA\models_X \phi \text{ and } \mA\models_X \psi\\
% % % \mA\models_X \phi\vee\psi &\Leftrightarrow& \mA\models_Y \phi \text{ and } \mA\models_Z \psi \text{ for some }Y\cup Z=X\\
% % % \mA \models_X \exists x \psi &\Leftrightarrow& \mA \models _{X(F/x)} \psi \text{ for some } F\colon X\to A\\
% % % \mA \models_X \forall x\psi&\Leftrightarrow& \mA \models _{X(A/x)} \psi\\
% % % \mA \models_X N^m_n \vec x_1\dots \vec x_m \alpha_1\dots \alpha_m \psi &\Leftrightarrow& \mA \models_Y\psi\\
% % % \multicolumn{3}{l}{\quad\text{\parbox[t]{13cm}{where $Y=X[A/\vec x_1\dots\vec x_m][F_1/\alpha_1]\dots[F_m/\alpha_m]$ and $F_i:X[A/\vec x_1\dots\vec x_m]\to\{\bot,\top\}$ is a $\{\vec x_1\dots\vec x_{i-1}\vec x_{i+1}\dots\vec x_m\}$-independent function for all $i\in\{1,\dots,m\}$.}}}
% % % \end{array}\]
% % % 
% % % Note that in the last case the functions $F_i$ only have to be independent of the variables universally quantified in rows $1,\dots,i-1,i+1,\dots,m$ of the POC but they may depend on variables quantified before the POC.
% % % 
% % % If $\phi$ is a sentence we usually just write $\mA\models \phi$ instead of $\mA\models_{\{\emptyset\}} \phi$.
% % % \end{definition}
% % % 
% % % \begin{definition}[Single-assignment semantics of \fopocp]\label{semantics fopocp single}
% % % \todopl{non-team semantics for POC}
% % % \end{definition}
% % % 
% % % \begin{proposition}
% % % Let $\phi\in\fopocp$, $\mA$ a structure and $X$ a team. Then
% % % \[\mA\models_X \phi \quad\text{iff}\quad \mA\models_s \phi\text{ for all $s\in X$},\]
% % % i.e.~the team semantics of $\fopocp$ (\cref{semantics fopocp}) is equivalent to the usual single-assignment semantics (\cref{semantics fopocp single}).
% % % \end{proposition}
% % % \begin{proof}
% % % \todopl{prove}
% % % \end{proof}
% % % 
% % % 
% % % \begin{remark}\label{poc-semantics-literature}
% % % \todopl{Lauri writes: our non-team POCs are equivalent with the versions from the literature}
% % % \end{remark}
% % % 
% % % 
% % % 
% % % % \todopl{free variables are first-order only?}
% % % 
% % % % \begin{definition}\label{Boolean-in-dep}
% % % % Let $\beta_1,\dots,\beta_n,\alpha$ Boolean variables and $x_1,\dots,x_m$ first-order variables. Then
% % % % \[\dep[x_1,\dots,x_m,\beta_1,\dots,\beta_n,\alpha]\]
% % % % is defined as a shorthand for
% % % % \[\forall u_1\forall u_1'\dots\forall u_n\forall u_n'\,\left(\bigwedge ...\dep[x_1,\dots,x_m,\beta_1,\dots,\beta_n,\alpha].\]
% % % % \end{definition}
% % % % The meaning of...
% % % 
% % % \begin{theorem}[0-1-law]\label{0-1-law}
% % % \todopl{write down}
% % % \end{theorem}
% % % \begin{proof}
% % % \cite[Theorem~10]{hesetu08} \todopl{comment on the source of 0-1-law for \fopocp}
% % % \end{proof}
% % % 
% % % \begin{definition}\label{reso}
% % % $\reso$ is the set of all $\eso$-formulas which do not contain any relation variable applications inside the scope of existential quantifiers.
% % % 
% % % \todopl{this ESO fragment is equivalent to \bbd. unfortunately, imo we have to redo the full $\pocfo\equiv \snp$ proof and then some more to prove this. the question is whether we want to have this at all. after all, this \eso fragment does not seem too natural. maybe everyone can write their thoughts about this here.}
% % % \end{definition}
% % % 
% % % \todopl{define \snp}




\section{Equivalences}
% \texorpdfstring{Equivalences between \bd fragments and \fopocp fragments}{Equivalences between BD fragments and FO(POC+) fragments}

% For proof technincal reasons we will now define the so called \emph{changed semantics} for \fopocp. The only difference to \cref{semantics fopocp} is the way we define semantics for the partial ordered connective. For the changed semantics we define that
% \[
% \mA \models_X N^m_n \vec x_1\dots \vec x_m \alpha_1\dots \alpha_m \psi \quad\Leftrightarrow\quad \mA \models_Y\psi
% \]
% where $Y=X[A/\vec x_1\dots\vec x_m][F_1/\alpha_1]\dots[F_m/\alpha_m] \text{ and } F_i:X[A/\vec x_1\dots\vec x_m]\to\{\bot,\top\}$ is a $\dom {X[A/\vec x_1\dots\vec x_m]}\setminus\{\vec x_i\}$ independent function. Notice that in the changed semantics the value of $\alpha_i$ is completely determined by the values of the variables $\vec x_i$, whereas in the normal semantics the value of $\alpha_i$ is determined by the values of the variables $\vec x_i$ with the values of the variables from $\dom X\setminus \{\vec x_i\}$. \todojv{ seminus needed if we reuse variables}

%\begin{definition}\label{changed-semantics}
%\todopl{define changed semantics}
%\end{definition}

% \begin{definition}\label{semantics-invariant}
% Let $\phi \in \fopocp$.
% Then we say that $\phi$ is \emph{semantics-invariant} if for all structures $\mA$ and teams $X$ with $\fr{\phi}\subseteq \dom{X}$ it holds that
% \[\mA\models_X \phi \quad\text{iff}\quad \mA\models_X' \phi.\]
% \end{definition}


% \begin{lemma}\label{changed-semantics-not-matter}
% Let
% \[\phi\,\dfn\ 
% \poc[ccccccc]{
% \forall y'_1&\dots&\forall y'_k&\forall x_{11}&\dots&\forall x_{1n}&\exists \alpha_1\\
% \vdots&&\vdots&\vdots&&\vdots&\vdots\\
% \forall y'_1&\dots&\forall y'_k&\forall x_{m1}&\dots&\forall x_{mn}&\exists \alpha_m}
% \left(\bigwedge_{i=1}^k y_i'=y_i\ \to\, \psi\right),\]
% a $\fopocp$-formula, where $\psi \in\fopocp$ and $\psi$ is semantics-invariant under $\{y_1,\dots,y_k,y_1',\dots,y'_k,x_{11},\dots,x_{mn}\}$.
% % Further let $\mA$ a structure and $X$ a team with $\fr{\phi}\subseteq \dom{X}$.
% Then $\phi$ is semantics-invariant under $\{y_1,\dots,y_k\}$.
% \end{lemma}
% \begin{proof}
% \end{proof}




% \begin{lemma}
% Let $\phi \in \fopocp$ be a sentence. Then there is a sentence $\phi'\in\fopocp$ such that for all structures $\mA$ it holds that $\mA\models' \phi$ iff $\mA\models\phi'$.
% \end{lemma}


\begin{theorem}\label{bbd-fopocp}
$\bbd \equiv \fopocp$
\end{theorem}
\begin{proof}
For the direction $\bbd \leqq \fopocp$ it is enough to show $\bbd\ff\leqq\fopocp$, by \cref{d-df}. Hence, we inductively define a translation $\phi\mapsto \phi'$ from $\bbd\ff$ to $\fopocp$. Therefore we assume w.l.o.g.~that no variable name is quantified more than once in $\phi$. For literals the translation is the identity. The other cases are translated as follows:
\[\begin{array}{rcl}
\psi \diamond \theta & \mapsto & \poc[c]{A \\ B} (\psi^* \diamond \theta^*)\\[2ex]
& \multicolumn{2}{l}{\text{for all $\diamond\in\{\wedge,\vee\}$}}\\[2ex]
\exists x \psi & \mapsto &  \exists x \poc[c]{A  } \psi^* \\[2ex]
\forall x \psi & \mapsto &  \poc[c]{A  } \forall x\psi^* \\[2ex]
\exists \alpha \dof{x_1,\dots,x_n}\,\psi & \mapsto &  \poc[c]{A \\ \forall u_1\dots\forall u_n\exists \alpha}\big((\bigwedge_{i=1}^n u_i=x_i)\to\psi^*\big)
\vspace*{-1ex}
\end{array}\]
where $\psi' = \poc{A}\psi^*$,\; $\theta' = \poc{B}\theta^*$ and we identify the absence of a partially-ordered connective with the empty POC $\poc{\,}$.

\begin{claim}\label{bbd-fopocp-bbd}
For all sentences $\phi\in\bbd\ff$ and all structures $\mA$,
\[\mA \models \phi \quad\text{iff}\quad \mA \models \phi'.\]
\end{claim}
\begin{namedproof}{\cref*{bbd-fopocp-bbd}}
First note that for $\phi \in \rbd\ff$, i.e.~if there is no $\exists \alpha\dof{x_1,\dots,x_n}$ within the scope of a $\exists x$, it holds that $\phi'\in\pocfo$ because in this case the only translation in which a partially-ordered connective occurs inside a translated formula instead of in its beginning -- namely the translation of $\exists x \psi$ -- cannot occur with a backslashed Boolean quantifier inside, by definition of $\rbd\ff$.

In this case the claimed equivalence holds since for each subformula $\exists\alpha\dof{x_1,\dots,x_n} \psi$ of $\phi$ there is a row $\poc{\forall u_1\dots\forall u_n\exists \alpha}$ in the POC and $\alpha$ occurs only inside $\psi^*$ -- where the variables $u_1,\dots,u_n$ are unified with $x_1,\dots,x_n$ and hence the determination of $\alpha$ by $u_1,\dots,u_n$ means that $\alpha$ is in fact determined by $x_1,\dots,x_n$.

In the case $\phi\notin\rbd\ff$ note that each partially-ordered connective in $\phi'$ occurs either in the beginning of the formula or directly below an existential first-order quantifier, i.e.~in the form $\exists x \poc{A}\psi^*$. In the latter case the POC is \emph{parameterized} by the assignments to variables that are free in $\poc{A}\psi^*$, i.e.~for each row $\poc{\forall u_1\dots\forall u_n\exists\alpha}$ in the POC the value of $\alpha$ may depend on all variables that are already bound when the POC is evaluated. This, however, does not violate the equivalence since, by definition of $\bbd\ff$, the universally quantified variables that are already bound must be among $x_1,\dots,x_n$ and hence $\alpha$ may depend on them (or, more precisely, their copies which are then unified) anyways.
\end{namedproof}

For the direction $\fopocp \leqq \bbd$ we inductively define a translation as follows.
For literals the translation is the identity. For first-order quantifiers as well as conjunction and disjunction it is defined in the canonical way.
Finally, partially-ordered connectives are translated by
\begin{multline*}
\phi\dfn
\poc[cccc]{
\forall x_{11}&\dots&\forall x_{1n}&\exists \alpha_1\\
\vdots&&\vdots&\vdots\\
\forall x_{m1}&\dots&\forall x_{mn}&\exists \alpha_m}
\psi \quad \mapsto\\
\forall x_{11}\dots\forall x_{1n}\dots \forall x_{m1}\dots\forall x_{mn}\exists \alpha_1\dots \exists \alpha_m \left(\bigwedge_{i=1}^m \dep[y_1,\dots,y_k,x_{i1},\dots,x_{in},\alpha_i]\ \wedge\ \psi\right)
\end{multline*}
where $\fr{\phi}=\{y_1,\dots,y_k\}$ and we assume that no variable name is requantified.
Note that $\alpha_1,\dots,\alpha_m$ may (implicitly) depend on Boolean variables, say $\gamma_1,\dots,\gamma_\ell$, that are free in $\phi$. However, the last assumption ensures that $\alpha_1,\dots,\alpha_m$ may depend on the first-order variables by which $\gamma_1,\dots,\gamma_\ell$ are determined and therefore we do not need to make the dependence on $\gamma_1,\dots,\gamma_\ell$ explicit.
\end{proof}



\begin{corollary}\label{rbd-pocfo}
$\rbd \equiv \pocfo$ % \equiv \reso$
\end{corollary}
\begin{proof}
% The equivalence $\rbd\equiv \pocfo$
This follows directly from the proof of \cref{bbd-fopocp} since the translations in that proof preserve the properties that distinguish $\rbd$ from $\bbd$ and $\pocfo$ from $\fopocp$.

% The equivalence $\pocfo \equiv \reso$ follows from ...
\end{proof}


\begin{corollary}\label{abd-pocqf}
$\abd \equiv \pocqf \equiv \snp$
\end{corollary}
\begin{proof}
The first equivalence follows immediately from the proof of \cref{bbd-fopocp} -- as in \cref{rbd-pocfo}.

The second equivalence is due to \cite[Lemma~6]{hesetu08}.
\end{proof}


\begin{theorem}\label{bd-d}
$\bd \equiv \df$
\end{theorem}
\begin{proof}
%``$\leqq$'': 
$\bd \leqq \df$ holds by \cref{logic-inclusions}.

% Let $\psi$ be a \bd sentence. Obviously, $\psi$ is a sentence in \D where for every dependence atom $\dep[x_1,\dots,x_n,y]$ the determined variable $y$ is from a Boolean domain.

%``$\geqq$'': 
On the other hand let $x_1,\dots, x_n, y_1,\dots,y_m$ be first-order variables and
\[\Phi \dfn\forall x_1\dots \forall x_n \exists y_1\dots \exists y_m \big(\bigwedge_{i=1}^m \dep[x_{j_{i,1}},\dots, x_{j_{i,k_i}},y_i]\; \wedge\; \phi\big),\]
be an arbitrary \df sentence in the normal form for \D from \cite[p.~98]{va07},
where $\phi$ is a quantifier-free first-order formula.

Let $\alpha_1,\dots, \alpha_m$ be Boolean variables and $z_1,\dots,z_m$ be first-order variables and let
%Then $\Phi$ is equivalent to the \bd sentence
\[\begin{array}{lll}
\psi &\dfn &\forall x_1\dots \forall x_n \exists y_1\dots\exists y_m\Big(\phi\wedge \forall z_1\dots \forall z_m \exists \alpha_1\dots \exists \alpha_m\\
&&\bigwedge\limits_{i=1}^m \big(\dep[x_{j_1},\dots,x_{j_i},z_i,\alpha_i]\wedge (z_i=y_i \leftrightarrow \alpha_i) \big) \Big).
\end{array}\]
be the translation of $\Phi$.

\begin{claim}\label{bd-d-claim}
Let \mA be a structure. Then it holds that \[\mA \models_{X} \Phi \text{ iff } \mA \models_{X} \psi.\]
\end{claim}
\begin{namedproof}{\cref*{bd-d-claim}}
It is enough if we can show, that the two formulae

\[\begin{array}{lll}
\tilde\Phi &\dfn &\bigwedge_{i=1}^m \dep[x_{j_1},\dots, x_{j_i}, y_i]\text{ and}\\
%\text{and}&&\\
\tilde\psi &\dfn &\forall z_1 \dots \forall z_m \exists \alpha_1 \dots \exists \alpha_m (\bigwedge_{i=1}^{m}\dep[x_{j_1},\dots, x_{j_i},z_i,\alpha_i] \wedge (y_i = z_i \leftrightarrow \alpha_i))
\end{array}\]
are equivalent.

Let $X$ be a team with $\dom{X} = \{x_1,\dots,x_n,y_1,\dots,y_m\}$ and
\[
\mA \models_{X} \tilde\Phi
\]
%By downwards closure, we can assume, that there are no double assignments in $X$.
%We have to show that $\mA \models_{X} \tilde\psi$.
Let $Y$ be the duplicated team for every variable $z_i$, i.e.
%For every value in $A$ of $z_i$ the team $X$ is duplicated. 
Let $A = |\mA| $, and $Y \dfn X(A/z_1)\dots(A/z_m)$.
% then that means
%\[
%\mA \models_{X} \tilde\Phi \text{ iff } \mA \models_{Y} \exists \alpha_1 \dots \exists \alpha_m (\bigwedge_{i=1}^{m} \dep[x_{j_1},\dots,x_{j_i},z_i,\alpha_i] \wedge (z_i = y_i \leftrightarrow \alpha_i)).
%\]

Let the function $F: X \to \{0,1\}$ be defined as follows
\[
F((\vec x,a_i),(\vec y, a_j),(\vec z, a_k)) = f(a_{k_1},\dots,a_{k_m},a_{j_1},\dots,a_{j_m})
\]
where
\begin{align*}
(\vec x, a_i) &\dfn \{x_1,a_{i_1}\},\dots,\{x_n,a_{i_n}\},\\
(\vec y, a_j) &\dfn \{y_1,a_{j_1}\},\dots,\{y_m,a_{j_m}\},\\
(\vec z, a_k) &\dfn \{z_1,a_{k_1}\},\dots,\{z_m, a_{k_m}\},\\
f(a_{k_1},\dots, a_{k_m}, a_{j_1},\dots, a_{j_m}) &\dfn \begin{cases} 
0 \text{ iff } a_{k_l} \neq a_{j_l}\\
1 \text{ iff } a_{k_l} = a_{j_l}
\end{cases}
\end{align*}

 and $Z \dfn Y(F/\alpha_1)\dots (F/\alpha_m)$. Then the $F$ gives the choice of the $\alpha_i$.
Since $f(\vec a_k, \vec a_j)$ is $1$ or $0$ iff the values of $z_i$ and $y_i$ are equal or not equal respectively, the second condition $z_i = y_i \leftrightarrow \alpha_i$ holds. In particular that means
\[
\mA \models_{Z} \bigwedge_{i=1}^{m} (z_i = y_i \leftrightarrow \alpha_i).
\]
And since $\mA \models_{X} \tilde \Phi$ we have that if $\vec x_i = \vec x_j \rightarrow y_i = y_j$. The team $Y$ is the duplication of $X$ for the variables $z_1,\dots,z_m$, hence for $Y$ it also holds that $\vec x_i = \vec x_j \rightarrow y_i = y_j$. Together with $z_i = y_i \leftrightarrow \alpha_i$ it follows, that $(\vec x_i,z_i) = (\vec x_j,z_j) \rightarrow \alpha_i = \alpha_j$ and thus
\[
\mA \models_{Z} \bigwedge_{i =1}^{m} \dep[x_{j_1},\dots,x_{j_i},z_i,\alpha_i].
\]
Altogether we have
\[
\begin{array}{lll}
&\mA &\models_{Z}\bigwedge_{i=1}^{m} \dep[x_{j_1},\dots,x_{j_i},z_i,\alpha_i] \wedge (z_i = y_i \leftrightarrow \alpha_i)\\
\Leftrightarrow&\mA &\models_{Y}  \exists \alpha_1 \dots \exists \alpha_m (\bigwedge_{i=1}^{m} \dep[x_{j_1},\dots,x_{j_i},z_i,\alpha_i] \wedge (z_i = y_i \leftrightarrow \alpha_i))\\
\Leftrightarrow &\mA &\models_{X} \tilde \psi.
\end{array}
\]

On the other hand let \mA be a structure and $X$ be a team with
\[
\mA \models_{X} \tilde\psi.
\]
Again let $Y\dfn X(A/x_1)\dots(A/z_m)$. Then we have
\[
\mA \models_{Y}\exists z_1\dots\exists z_m \bigwedge_{i=1}^{m}(\dep[z_{j_1},\dots,z_{j_i},z_i,\alpha_i]\wedge (z_i = y_i \leftrightarrow \alpha_i))
\]
%\todoje{Incomplete! To be continued...}
\end{namedproof}
~
%(Greek letters: Boolean variables; Latin letters: first-order variables)
\end{proof}
\todoje{indices are wrong}

Note that this also gives a normal form theorem: Every \bd sentence can be equivalently expressed in the form
\begin{multline*}
\forall x_1\dots \forall x_n \,\exists y_1\dots \exists y_m \, \forall  z_1\dots\forall z_m\, \exists \alpha_1\dots \exists \alpha_m\\
\Big(\bigwedge_{i=1}^m \big(\dep[x_{j_{i,1}},\dots, x_{j_{i,k_i}}, z_i, \alpha_i]\ \wedge (z_i = y_i \leftrightarrow \alpha_i)\big)\wedge\ \phi\Big),
\end{multline*}
where $\phi$ is a quantifier-free first-order formula.

\todopl{normal forms for \rbd and \abd}


\section{Separations}


\begin{lemma}\label{abd closed}
Let $\mA$ be a model, $\mB$ a submodel of $\mA$ and $\phi$ a \abd-sentence.
\[
\text{If }\mA\models \phi \text{ then } \mB\models \phi.
\]
\end{lemma}
\begin{proof}
We have shown in \cref{abd-pocqf} that $\abd\equiv\snp$. The fact that the lemma holds for \snp can be proven by a simple inductive argument. The result can also be seen as a modification of \cite[Lemma~1.2]{barwise:applications}.
\end{proof}

\begin{proposition}\label{abd-rbd}
$\abd \lneqq \rbd$
\end{proposition}
\begin{proof}
It was stated in \cref{logic-inclusions} that $\abd\leqq \rbd$. Since by \cref{abd closed} the truth of a \abd sentence is preserved under submodels, it is enough to show that there is an $\rbd$ sentence for which the truth is not preserved under submodels. Clearly the following \rbd sentence stating that the domain of the model has at least two points suffices.
\[
\exists x \exists y \, x \neq y
\]
\end{proof}


\begin{definition}\label{equiv_L}
Let $\LL$ be a logic (or a fragment of a logic), $\tau$ a vocabulary and $\mA$, $\mB$ first-order 
structures over $\tau$. Then we write $\mA\simp_{\LL}\mB$ if and only if the implication 
$\mA\models \phi\Rightarrow\mB\models \phi$ holds for all sentences $\phi \in \LL$.
\end{definition}

Let $\mnfor$ denote the set of all sentences in $\pocfo$ which are of the
form $N^m_n\vec x_1\dots \vec x_m \alpha_1\dots\alpha_m\,\phi$, where
$\phi$ is a first-order formula with quantifier rank at most $r$.
We will next define an Ehrenfeucht-Fra\"{\i}ss\'{e} game that captures the truth preservation
relation $\mA\simp_{\mnfor}\mB$. This game is a straightforward modification of the 
corresponding game for the partially ordered connectives $D^m_n$ by Sevenster and
Tulenheimo \cite{setu06c}, which in turn is based on the EF game for first-order logic
with all partially ordered connectives, introduced by Sandu and V\"a\"an\"anen \cite{sava92}. 

\begin{definition}\label{ef game rbd}
Let $\mA$ and $\mB$ first-order structures over a vocabulary $\tau$ and let $m\geq 2$, 
$n\geq 1$ and $r\geq 0$. The \emph{$\mnfor$-Ehrenfeucht-Fra\"{\i}ss\'{e} ($\mnfor$-EF) game} 
$\efgmnr(\mA,\mB)$ with $N^m_n$-prefix and $r$ first-order rounds on $\mA$ and 
$\mB$ is played by two players, Spoiler and Duplicator, and it has two phases.
\medskip

\noindent {\bf Phase 1:}
\begin{itemize}
\item Spoiler chooses $n$-ary functions $f_1,\ldots,f_m: A^n\to\{\bot,\top\}$ on $A$. 
\item Duplicator answers by choosing $n$-ary functions $g_1,\ldots,g_m: B^n\to\{\bot,\top\}$ on $B$. 
\item Spoiler chooses $n$-tuples $\vec b_1,\ldots,\vec b_m\in B^n$. 
\item Duplicator answers by choosing $n$-tuples $\vec a_1,\ldots,\vec a_m\in A^n$ such that
for each $1\leq i\leq m$, $f_i(\vec a_i)=g_i( \vec b_i)$. If there are no tuples 
$\vec a_1,\ldots,\vec a_m\in A^n$ satisfying this condition, then Duplicator loses the the play 
of the game.
\end{itemize}
\noindent {\bf Phase 2:}
\begin{itemize}
\item Spoiler and Duplicator play the usual first-order EF-game of $r$ rounds
on the structures $(\mA,\vec a_1\ldots\vec a_m)$ and $(\mB,\vec b_1\ldots\vec b_m)$:
In each round $1\leq j\leq r$, Spoiler picks an element $c_j\in A$ (or $d_j\in B$), and
Duplicator answer by choosing an element $d_j\in B$ (or $c_j\in A$, respectively).
\end{itemize}
Duplicator wins the play of the game if and only if the mapping 
$\vec a_1\ldots\vec a_m c_1\ldots c_r\mapsto \vec b_1\ldots\vec b_m d_1\ldots d_r$
is a partial isomorphism $\mA\to\mB$.

We say that Duplicator has a winning strategy in the game if and only she has a 
systematic way of answering all possible moves of Spoiler such that using it she 
always wins the play. 
\end{definition}

We show next that the game $\efgmnr$ can be used for studying the truth preservation
relation $\simp_{\mnfor}$. This result is essentially the same as Proposition 12 in \cite{setu06c},
which in turn is a special case of Proposition 7 in \cite{sava92}. 

\begin{lemma}\label{ef char}
Let $\mA$ and $\mB$ first-order structures over a vocabulary $\tau$ and let
$m\geq 2$, $n\geq 1$ and $r\geq 0$. If Duplicator has a winning strategy in 
the game $\efgmnr(\mA,\mB)$, then $\mA\simp_{\mnfor}\mB$.
\end{lemma}
\begin{proof}
Assume that Duplicator has a winning strategy in the game $\efgmnr(\mA,\mB)$.
To prove $\mA\simp_{\mnfor}\mB$, assume that 
$\psi=N^m_n\vec x_1\dots \vec x_m \alpha_1\dots\alpha_m\,\phi$ is a sentence
of $\mnfor$ such that $\mA\models\psi$. Thus, there are functions $f_1,\ldots,f_m: A^n\to
\{\bot,\top\}$ such that for all $\vec a_1,\ldots,\vec a_m\in A^n$, $\mA\models_{s[\vec a,\vec f]}\psi$,  
where $s[\vec a,\vec f]$ is the assignment such that $s[\vec a,\vec f](\vec x_i)= \vec a_i$ 
and $s[\vec a,\vec f](\alpha_i)= f_i(\vec a_i)$ for $1\leq i\leq m$.

Let $g_1,\ldots,g_m: B^n\to\{\bot,\top\}$ be the answer given by Duplicator's winning strategy
in the play where $f_1,\ldots,f_m$ is the first move of Spoiler. 
It suffice to show that for all $\vec b_1,\ldots,\vec b_m\in B^n$, $\mB\models_{s[\vec b,\vec g]}\psi$.
Thus, let $\vec b_1,\ldots,\vec b_m\in B^n$ be
arbitrary $n$-tuples in $B$. Let $\vec a_1,\ldots,\vec a_m\in A^n$ be the answer given by 
Duplicator's winning strategy when Spoiler's second move is $\vec b_1,\ldots,\vec b_m$.
By the definition of the game $\efgmnr$, Duplicator has then a winning strategy in the first-order 
EF game with $r$ rounds between the structures $(\mA,\vec a_1,\ldots,\vec a_m)$ and 
$(\mB,\vec b_1,\ldots,\vec b_m)$. By the standard EF theorem, it follows that 
$(\mA,\vec a_1,\ldots,\vec a_m)$ and $(\mB,\vec b_1,\ldots,\vec b_m)$ satisfy the
same $\fo_r$-sentences. Note further that 
$f_1(\vec a_1)=g_1( \vec b_1)\ldots, f_m(\vec a_m)=g_m( \vec b_m)$ by the condition
governing the choice of $\vec b_1,\ldots,\vec b_m$, whence  
$(\mA,\vec a_1,\ldots,\vec a_m, f_1(\vec a_1),\ldots,f_m(\vec a_m))$ and 
$(\mB,\vec b_1,\ldots,\vec b_m, g_1(\vec b_1),\ldots,g_m(\vec b_m))$ are also equivalent 
with respect to all sentences of $\fo_r$ (extended with Boolean constants). In particular,
since $\mA\models_{s[\vec a,\vec f]}\psi$, we have $\mB\models_{s[\vec b,\vec g]}\psi$, as desired.
\end{proof}

\begin{corollary}\label{pocfo def}
Let $\tau$ be a vocabulary, and let $K$ be a class of $\tau$-structures. If for all
$m\geq 2$, $n\geq 1$ and $r\geq 0$ there are $\tau$-structures $\mA$ and $\mB$
such that $\mA\in K$, $\mB\not\in K$ and Duplicator has a winning strategy in
$\efgmnr(\mA,\mB)$, then $K$ is not definable in $\pocfo$.
\end{corollary}
\begin{proof}
We prove the contraposition of the claim. Thus,
assume that $K$ is definable in $\pocfo$. Then there is a sentence $\psi$
of the form $N^m_n\vec x_1\dots \vec x_m \alpha_1\dots\alpha_m\,\phi$ such that
$K=\{\mA\mid\mA\models\psi\}$. Let $r$ be the quantifier rank of $\phi$. Then 
by \cref{ef char}, there are no structures $\mA\in K$ and $\mB\not\in K$ such that Duplicator 
has a winning strategy in the game $\efgmnr(\mA,\mB)$.  
\end{proof}

\begin{theorem}\label{rbd-bbd}
$\rbd \lneqq \bbd$
\end{theorem}
\begin{proof}
We show that non-connectivity of graphs is definable in $\bbd$, but not in $\rbd$.
Note first that a graph $\mA=(A,E^\mA)$ is not connected if and only if there is a 
subset $U\subseteq A$ such that $U$ and $A\setminus U$ are non-empty, and
there are no edges $(a,b)\in E^\mA$ between  $U$ and $A\setminus U$. This can 
be expressed by the $\bbd$-sentence
\[\begin{array}{llll}
   \exists u\exists v\forall x\forall y \exists\alpha\exists\beta \big(  & &  \dep[x,\alpha] \land \dep[y,\beta] &\arraycomment{There are two relations\dots}\\
   & \land & (x=y\to (\alpha\leftrightarrow\beta)) &\arraycomment{\dots which are equal\dots}\\
   & \land & (x=u\to \alpha) \land (x=v\to \lnot\alpha) &\arraycomment{\dots and contain $u$ but not $v$.}\\
   & \land & (\alpha\land\lnot\beta\to \lnot Exy)\, \big). &\arraycomment{\parbox[t]{5.5cm}{If $x$ is in the relations but $y$ is not then there is no edge between $x$ and $y$.}}
\end{array}\]

We use \cref{pocfo def} to prove that non-connectivity is not definable
in $\pocfo$. By \cref{rbd-pocfo}, it then follows that non-connectivity is not definable
in $\rbd$. 
Let us fix the number of rounds $r\geq 0$, the arity $n\geq 1$ and the
number of rows $m\geq 2$, and consider the game $\efgmnr$. Let $\mA=(A,E^\mA)$ 
and $\mB=(B,E^\mB)$ be
the graphs such that 
\begin{itemize}
\item $B=\{u_1,\ldots, u_k\}$, 
\item $A=B\cup \{v_1,\ldots,v_k\}$,
\item $E^\mB=\{(u_i,u_j)\mid |i-j|=1\}\cup \{(u_1,u_k),(u_k,u_1)\}$, 
\item $E^\mA=E^\mB\cup\{(v_i,v_j)\mid |i-j|=1\}\cup \{(v_1,v_k),(v_k,v_1)\}$.
\end{itemize}
Thus, $\mB$ is a cycle of length $k$, and $\mA$ is the disjoint union of
two cycles of length $k$. In particular, $\mA$ is not connected, but $\mB$ is 
connected. We will now show that if $k$ is large enough, then Duplicator has a winning 
strategy in the game $\efgmnr(\mA,\mB)$.

Let $f_1,\ldots, f_m: A^n\to\{\bot,\top\}$ be the first move of Spoiler in the game. 
Duplicator's answer is then $g_1,\ldots, g_m: B^n\to\{\bot,\top\}$, where for each 
$1\leq i\leq m$, $g_i$ is the restriction $f_i\upharpoonright B$ of $f_i$ to the set $B$. 
In the next move Spoiler picks tuples 
$\vec b_1,\ldots\vec b_m\in B^m$. Now Duplicator can simply answer by choosing
the same tuples: let $\vec a_i=\vec b_i$ for each  $1\leq i\leq m$. Clearly
the requirement $f_i(\vec a_i)=g_i(\vec b_i)$ is then satisfied.
The game continues after this as the first-order EF-game with $r$ rounds
on the structures $(\mA,\vec a_1\ldots\vec a_m)$ and $(\mB,\vec b_1\ldots\vec b_m)$.
Since the mapping $\vec a_1\ldots\vec a_m\mapsto\vec b_1\ldots\vec b_m$
respects distances between nodes in the graphs $\mA$ and $\mB$, a standard 
argument shows that Duplicator has a winning strategy in the rest of the game,
provided that $k$ is big enough. 

More precisely, assume that $k > m \cdot n \cdot 2^r$, and let $a_1,\ldots a_{mn}$ be the
components of the tuples $\vec a_1,\ldots,\vec a_m$. Then $d^\mA(a_i,a_j)=d^\mB(a_i,a_j)$ 
for all $i,j\in\{1,\ldots,mn\}$, where $d^\mA(u,v)$ ($d^\mB(u,v)$) is the distance between the
nodes $u$ and $v$ in the graph $\mA$ ($\mB$, respectively).  Furthermore, by the assumption
on $k$, there are $i,j\in \{1,\ldots,mn\}$ such that $d^\mA(a_i,a_j)>2^r$ and there is no
$l\in\{1,\ldots,mn\}$ such that $a_l$ is inbetween $a_i$ and $a_j$ on the cycle $B$. 
\end{proof}

\tikzstyle{place}=[circle,draw=black!100,fill=white!100,thick]
\begin{figure}
\begin{center}
\begin{minipage}[b]{0.46\textwidth}
\begin{center}
\begin{tikzpicture}[-,>=stealth',shorten >=1pt,auto,node distance=1.8cm, thick]
        \draw[thick] (0:3cm) arc (0:105:3cm);
        \draw[dotted] (105:3cm) arc (105:360:3cm);
        \node[circle,minimum size=4cm](A){}; 
        \node[place,] at (A.45)         (u1)            [label=above right:{$u_1$}] {$s_1$}; 
        \node[place] at (A.65)  (u2)            [label=above right:{$u_2$}] {$s_2$}; 
        \node[place] at (A.85)  (u1)            [label=above right:{$u_3$}] {}; 
        \node[place] at (A.105)         (u1)            [label=above right:{$u_4$}] {}; 
        \node[place] at (A.25)  (uk)            [label=above right:{$u_k$}] {}; 
        \node[place] at (A.5)   (uk1)           [label=above right:{$u_{k-1}$}] {}; 
\end{tikzpicture}
\end{center}
\end{minipage}
\hspace{0.04\textwidth}
\begin{minipage}[b]{0.48\textwidth}
\begin{center}
\begin{tikzpicture}[-,>=stealth',shorten >=1pt,auto,node distance=1.8cm, thick] 
        \draw[thick] (0:3) arc (0:105:3cm);
        \draw[dotted] (105:3) arc (105:195:3cm);
        \draw[thick] (195:3) arc (195:245:3cm);
        \draw[dotted] (245:3) arc (245:360:3cm);
        \node[circle,minimum size=4cm](B){}; 
        \node[place] at (B.45)  (v1)            [label=above right:{$v_1$}] {}; 
        \node[place] at (B.65)  (v2)            [label=above right:{$v_2$}] {$s_5$}; 
        \node[place] at (B.85)  (v1)            [label=above right:{$v_3$}] {}; 
        \node[place] at (B.105)         (v1)            [label=above right:{$v_4$}] {}; 
        \node[place] at (B.25)  (vk)            [label=above right:{$v_k$}] {}; 
        \node[place] at (B.5)           (vk1)   [label=above right:{$v_{k-1}$}] {}; 
        \node[place] at (B.210)         (vl)            [label=below left:{$v_l$}] {$s_3$}; 
        \node[place] at (B.230)         (vl1)           [label=below left:{$v_{l+1}$}] {$s_4$}; 
\end{tikzpicture}
\end{center}
\end{minipage}
\end{center}
\caption{The structure \mA where spoiler chooses at first $s_1$ and duplicator answers in \cref{fig_mB} with $d_1$. Next spoiler chooses $s_2$ duplicator answers with the corresponding $d_2$ and so on.}
\label{fig_mA}
\end{figure}

\begin{figure}
\begin{center}
\begin{tikzpicture}[-,>=stealth',shorten >=1pt,auto,node distance=1.8cm, thick]
        \draw[thick] (0:3cm) arc (0:105:3cm);
        \draw[dotted] (105:3cm) arc (105:195:3cm);
        \draw[thick] (195:3cm) arc (195:245:3cm);
        \draw[dotted] (245:3cm) arc (245:300:3cm);
        \draw[thick] (300:3cm) arc (300:330:3cm);
        \draw[dotted] (330:3cm) arc (330:360:3cm);
        \node[circle,minimum size=4cm](A){}; 
        \node[place] at (A.45)  (u1)            [label=above right:{$u_1$}] {$d_1$}; 
        \node[place] at (A.65)  (u2)            [label=above right:{$u_2$}] {$d_2$}; 
        \node[place] at (A.85)  (u1)            [label=above right:{$u_3$}] {}; 
        \node[place] at (A.105)         (u1)            [label=above right:{$u_4$}] {}; 
        \node[place] at (A.25)  (uk)            [label=above right:{$u_k$}] {}; 
        \node[place] at (A.5)   (uk1)           [label=above right:{$u_{k-1}$}] {}; 
        \node[place] at (A.210)         (ul)            [label=below left:{$u_l$}] {$d_3$}; 
        \node[place] at (A.230)         (ul1)           [label=below left:{$u_{l+1}$}] {$d_4$}; 
        \node[place] at (A.315)         (ur)            [label=below right:{$u_r$}] {$d_5$}; 
\end{tikzpicture}
\end{center}
\caption{The structure \mB where duplicator answers on $s_1$ from \cref{fig_mA} with $d_1$ then on $s_2$ with $d_2$ and so on.}
\label{fig_mB}
\end{figure}

\todoje{Layout of the pictures is not good, i'm trying to find a better one to display the choices of spoiler and duplicator.}

\begin{proposition}\label{rbd-bd}
$\bbd \lneqq \bd$
\end{proposition}
\begin{proof}
By \cref{rbd-pocfo} and \cref{0-1-law} we know that \bbd has 0-1-law. Hence it cannot express even cardinality of the domain. But by \cref{bd-d} and \cite[Chapter~4.1]{va07} this property is definable in \bd.
\end{proof}

\todopl{write some rationale for stating the next remark}

\begin{remark}\label{bd-emso}
\begin{enumerate}
\item\label{emso-bbd} $\emso\nleqq \bbd$ and
\item\label{abd-emso} $\abd \nleqq \emso$.
\end{enumerate}
\end{remark}
\begin{proofsketch}
% It was shown in the proof of \cref{rbd-bbd} that non-connectivity of a graph is not definable in \rbd. We will show that non-connectivity is definable in $\emso$. This will prove that $\emso\nleqq \rbd$.
% 
% It is well known that a graph is not connected if and only if the domain of the graph can be partitioned in two non empty sets in a way that there are no edges between the partitions. Hence the following $\emso$ sentence defines non-connectivity:
% 
% \[
% \exists X ( \exists x \exists y ( X(x)\wedge \neg X(y)) \wedge \forall x\forall y (X(x)\wedge \neg X(y)\rightarrow \neg E(x,y)))
% \]
% 
% \todopl{Jonni writes about unconnectivity in $\emso$ but not in \rbd}
For part \enumref{emso-bbd} note that from the proof of \cref{rbd-bd} it follows that $\bbd$ has 0-1-law. On the other hand it was shown by Kaufmann that $\emso$ does not have 0-1-law \cite{ka88}.

For \enumref{abd-emso} note that the non-regular language
\[\set{a^n\,b^n}{$n\in \N$}\]
is definable by a $\pocfo$ formula but not by an $\emso$ formula since $\emso$ over word structures can only define regular languages.
\end{proofsketch}

\todopl{monadic versions of \pocfo, \pocqf, \rbd, \abd, \bd}

\begin{remark}
k-$\eso \equiv $k-$\bd$
\end{remark}
\begin{proof}
\todopl{k-ary fragments are the same. translate from \bd to \eso via \bd\ff.}
\end{proof}


\section{Conclusion}

\todopl{definability of common properties: e.g. infinity in \bbd or \rbd (it is not definable in \abd)}


\nocite{va07, hesetu08}

